Efficient Kernelized Learning in Polyhedral Games Beyond Full-Information: From Colonel Blotto to Congestion Games

We examine the problem of efficiently learning coarse correlated equilibria (CCE) in polyhedral games, that is, normal-form games with an exponentially large number of actions per player and an underlying combinatorial structure. Prominent examples of such games are the classical Colonel Blotto and congestion games. To achieve computational efficiency, the learning algorithms must exhibit regret and per-iteration complexity that scale polylogarithmically in the size of the players' action sets. This challenge has recently been addressed in the full-information setting, primarily through the use of kernelization. However, in the case of the realistic, but mathematically challenging, partial-information setting, existing approaches result in suboptimal and impractical runtime complexity to learn CCE. We tackle this limitation by building a framework based on the kernelization paradigm. We apply this framework to prominent examples of polyhedral games -- namely the Colonel Blotto, graphic matroid and network congestion games -- and provide computationally efficient payoff-based learning algorithms, which significantly improve upon prior works in terms of the runtime for learning CCE in these settings.

==> math-commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

% \usepackage{amsmath,amsfonts,bm}
\usepackage{multirow,array}
\usepackage{diagbox}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}

\newcommand{\matA}{\mat{A}}
\newcommand{\vecb}{\vec{b}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
% \def\vmu{{\bm{\mu}}}
% \def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
% \def\mA{{\bm{A}}}
% \def\mB{{\bm{B}}}
% \def\mC{{\bm{C}}}
% \def\mD{{\bm{D}}}
% \def\mE{{\bm{E}}}
% \def\mF{{\bm{F}}}
% \def\mG{{\bm{G}}}
% \def\mH{{\bm{H}}}
% \def\mI{{\bm{I}}}
% \def\mJ{{\bm{J}}}
% \def\mK{{\bm{K}}}
% \def\mL{{\bm{L}}}
% \def\mM{{\bm{M}}}
% \def\mN{{\bm{N}}}
% \def\mO{{\bm{O}}}
% \def\mP{{\bm{P}}}
% \def\mQ{{\bm{Q}}}
% \def\mR{{\bm{R}}}
% \def\mS{{\bm{S}}}
% \def\mT{{\bm{T}}}
% \def\mU{{\bm{U}}}
% \def\mV{{\bm{V}}}
% \def\mW{{\bm{W}}}
% \def\mX{{\bm{X}}}
% \def\mY{{\bm{Y}}}
% \def\mZ{{\bm{Z}}}
% \def\mBeta{{\bm{\beta}}}
% \def\mPhi{{\bm{\Phi}}}
% \def\mLambda{{\bm{\Lambda}}}
% \def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}


\newcommand{\calA}{\ensuremath{\mathcal{A}}}
\newcommand{\calB}{\ensuremath{\mathcal{B}}}
\newcommand{\calC}{\ensuremath{\mathcal{C}}}
\newcommand{\calD}{\ensuremath{\mathcal{D}}}
\newcommand{\calE}{\ensuremath{\mathcal{E}}}
\newcommand{\calF}{\ensuremath{\mathcal{F}}}
\newcommand{\calG}{\ensuremath{\mathcal{G}}}
\newcommand{\calH}{\ensuremath{\mathcal{H}}}
\newcommand{\calI}{\ensuremath{\mathcal{I}}}
\newcommand{\calJ}{\ensuremath{\mathcal{J}}}
\newcommand{\calK}{\ensuremath{\mathcal{K}}}
\newcommand{\calL}{\ensuremath{\mathcal{L}}}
\newcommand{\calM}{\ensuremath{\mathcal{M}}}
\newcommand{\calN}{\ensuremath{\mathcal{N}}}
\newcommand{\calO}{\ensuremath{\mathcal{O}}}
\newcommand{\calP}{\ensuremath{\mathcal{P}}}
\newcommand{\calQ}{\ensuremath{\mathcal{Q}}}
\newcommand{\calR}{\ensuremath{\mathcal{R}}}
\newcommand{\calS}{\ensuremath{\mathcal{S}}}
\newcommand{\calT}{\ensuremath{\mathcal{T}}}
\newcommand{\calU}{\ensuremath{\mathcal{U}}}
\newcommand{\calV}{\ensuremath{\mathcal{V}}}
\newcommand{\calW}{\ensuremath{\mathcal{W}}}
\newcommand{\calX}{\ensuremath{\mathcal{X}}}
\newcommand{\calY}{\ensuremath{\mathcal{Y}}}
\newcommand{\calZ}{\ensuremath{\mathcal{Z}}}



\newcommand{\vxstar}{\vx^*}
\newcommand{\vystar}{\vy^*}

\newcommand{\Amax}{\mat{A}_{\max}}
\newcommand{\Amin}{\mat{A}_{\min}}

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
%\newcommand{\Linv}{L_{\lambda_{\mathrm{inv}}}}
\newcommand{\R}{\mathbb{R}}
%\newcommand{\emp}{\tilde{p}}
%\newcommand{\lr}{\alpha}
%\newcommand{\reg}{\lambda}
%\newcommand{\rect}{\mathrm{rectifier}}
%\newcommand{\softmax}{\mathrm{softmax}}
%\newcommand{\sigmoid}{\sigma}
%\newcommand{\softplus}{\zeta}
%\newcommand{\KL}{D_{\mathrm{KL}}}
%\newcommand{\Var}{\mathrm{Var}}
%\newcommand{\standarderror}{\mathrm{SE}}
%\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}

% \DeclareMathOperator{\sign}{sign}
% \DeclareMathOperator{\Tr}{Tr}
% \let\ab\allowbreak

% \newtheorem{claim}[theorem]{Claim}
% \newtheorem*{nclaim}{Claim}

%%%%%% Paper specific commands
% \renewcommand{\diam}{\mathrm{diam}}
\newcommand{\metric}{\mathrm{d}}
\newcommand{\hausdorff}{\mathrm{d}_{\rmH}}
\newcommand{\size}{\mathrm{size}}
% \newcommand{\nm}[1]{\b{#1} - 1}
% \renewcommand{\sign}{\mathrm{sign}}
\renewcommand{\bar}[1]{\overline{#1}}


\newcommand{\tstar}{t^{\star}}

\newcommand{\autakia}[1]{``#1''}

\newcommand{\step}[1]{^{(#1)} }
\newcommand{\projoper}{\Pi_{\Delta}}
\newcommand{\projoperX}[1]{{\Pi_{\calX_{#1}}}}
\newcommand{\projoperY}[1]{{\Pi_{\calY_{#1}}}}
\newcommand{\projoperZ}[1]{{\Pi_{\calZ_{#1}}}}


% \renewcommand{\vv}[1]{\mathbf{#1}}
% \AtBeginDocument{\renewcommand{\vec}[1]{\mathbf{#1}}}

%%%%% New commands
% \include{mathcommands}

% \usepackage[urlcolor=blue]{hyperref}
% \usepackage{enumerate}
% \usepackage{amsmath}
% \usepackage{amsthm}
%\usepackage[short,nocomma]{optidef}
% \newtheorem{theorem}{Theorem}
% \newtheorem{lemma}{Lemma}

% \usepackage[lmargin=2cm, rmargin=2cm, tmargin=2cm, bmargin=2.5cm]{geometry}
% \usepackage{natbib}
% \bibliographystyle{unsrtnat}

%%%%%%%%%%%%%%%%%%%%Paper specific
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\px}{\bm{x}}
\newcommand{\pxhat}{\hat{\bm{x}}}
\newcommand{\pxtilde}{\tilde{\bm{x}}}

\newcommand{\py}{\bm{y}}
\newcommand{\pyhat}{\hat{\bm{y}}}
\newcommand{\pytilde}{\tilde{\bm{y}}}

\newcommand{\allagents}{i \in \calN}
\newcommand{\policy}[1]{\boldsymbol{\pi}_{{#1}}}
\newcommand{\adv}{\text{adv}}
\newcommand{\sign}{\mathrm{sign}}
\newcommand{\diag}{\mathrm{diag}}


\newcommand{\norm}[1]{\left\| #1 \right\|}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\lpref}[1]{\oldref{#1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand*\vell{\ensuremath{\boldsymbol\ell}}

\newcommand{\valpha}{\boldsymbol{\alpha} }
\newcommand{\vbeta}{\boldsymbol{\beta} }
\newcommand{\vgamma}{\boldsymbol{\gamma} }
\newcommand{\vdelta}{\boldsymbol{\delta} }
\newcommand{\vepsilon}{\boldsymbol{\epsilon} }
\newcommand{\vzeta}{\boldsymbol{\zeta} }
\newcommand{\veta}{\boldsymbol{\eta} }
\newcommand{\vtheta}{\boldsymbol{\theta} }
\newcommand{\viota}{\boldsymbol{\iota} }
\newcommand{\vkappa}{\boldsymbol{\kappa} }
\newcommand{\vlambda}{\boldsymbol{\lambda} }
\newcommand{\vmu}{\boldsymbol{\mu} }
\newcommand{\vnu}{\boldsymbol{\nu} }
\newcommand{\vxi}{\boldsymbol{\xi} }
\newcommand{\vomikron}{\boldsymbol{\omikron} }
\newcommand{\vpi}{\boldsymbol{\pi} }
\newcommand{\vrho}{\boldsymbol{\rho} }
\newcommand{\vsigma}{\boldsymbol{\sigma} }
\newcommand{\vtau}{\boldsymbol{\tau} }
\newcommand{\vypsilon}{\boldsymbol{\ypsilon} }
\newcommand{\vphi}{\boldsymbol{\phi} }
\newcommand{\vchi}{\boldsymbol{\chi} }
\newcommand{\vpsi}{\boldsymbol{\psi} }
\newcommand{\vomega}{\boldsymbol{\omega} }
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}

\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\dist}{dist}
\newcommand{\prox}{\mathrm{prox}}
\newcommand{\paren}[1]{\left(#1\right)}

\newcommand{\inprod}[2]{\left\langle#1,#2\right\rangle}
\newcommand{\mybrace}[1]{\left\{ #1 \right\}}

\newcommand{\mybracket}[1]{\left[ #1 \right]}

\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{amsmath}
\usepackage{bbm}
\usepackage{amsfonts}


%\theoremstyle{definition}  %
% \newtheorem{exercise}{Exercise}
% \newtheorem{claim}{Claim}
% \newtheorem{lemma}{Lemma}
% \newtheorem{conjecture}{Conjecture}
% \newtheorem{corollary}{Corollary}
% \newtheorem{proposition}{Proposition}
% \newtheorem{fact}{Fact}
% \newtheorem{assumption}{Assumption}
% \newtheorem{problem}{Problem}
% \newtheorem{question}{Question}
% \newtheorem{model}{Model}
% \theoremstyle{plain}
% \newtheorem{remark}{Remark}
% \newtheorem{example}{Example}
% \newtheorem{theorem}{Theorem}
% \newtheorem{observation}{Observation}

% \newtheorem{definition}{Definition}
% \newtheorem{openproblem}{Open Problem}

%\numberwithin{observation}{section}


%\numberwithin{claim}{section}
%\numberwithin{fact}{section}
%\numberwithin{lemma}{section}
%\numberwithin{proposition}{section}
%\numberwithin{theorem}{section}
%\numberwithin{corollary}{section}
%\numberwithin{definition}{section}
%\numberwithin{assumption}{section}

==> paper-specific-macros.tex <==
%Define behavior of the command with one parameter
% \newcommand{\proj1}[1]{\mathrm{Proj}_{#1}\left( #2 \right)}

%Define behavior of the command with two parameter
\newcommand{\projA}[1]{\mathrm{Proj}_{#1}}
\newcommand{\projB}[2]{\mathrm{Proj}_{#1}\left( #2 \right)}

%Define a new command with the desired name. It checks if parameter #2 exists; 
%if no, it invokes the first command definition for single parameter (\Seta), else it invokes the \Setb
\NewDocumentCommand\proj{ m g }{
  \IfNoValueTF{#2}{\projA{#1}}{\projB{#1}{#2}}
}

% \newcommand{\proj}[2]{\mathrm{Proj}_{#1}\left( #2 \right)}
% \newcommand{\proj}[1]{}

\newcommand{\attime}[1]{^{(#1)}}
% \renewcommand{\ve}{\mathbf{e}}
\usepackage{xspace}
\newcommand{\team}{\text{team}}
\newcommand{\hatpolicy}{\hat{\boldsymbol{\pi}}}
\newcommand{\GDmax}{$\textsc{GDmax}$\xspace}
\newcommand{\SGDmax}{$\textsc{ISNPG}$\xspace}
\newcommand{\AGDA}{$\textsc{AGDA}$\xspace}
\newcommand{\GDA}{$\textsc{GDA}$\xspace}
\newcommand{\SAGDA}{$\textsc{Stoch-AGDA}$\xspace}
\newcommand{\SGDA}{$\textsc{Stoch-GDA}$\xspace}
\newcommand{\REGVISMAX}{$\textsc{Vis-Reg-PG}$\xspace}


\newcommand{\IPGmax}{$\textsc{IPGmax}$\xspace}
\newcommand{\SIPGmax}{$\textsc{ISPNG}$\xspace}

\newcommand{\advnashpolicy}{\textup{\texttt{AdvNashPolicy}}\xspace}

\newcommand{\matP}[1]{\pr^{#1}}


%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% notation macros
\newcommand{\traj}{\tau}
\newcommand{\advparamspace}{\ensuremath{\mathcal{Y}}}
\newcommand{\importanceweight}[3]{\ensuremath{\omega_{t}(#1|#2, #3)}}
\newcommand{\advparam}{\ensuremath{\bm{\vy}}}
\newcommand{\lambdaest}{\ensuremath{\tilde{\vlambda}}}
\newcommand{\gradest}{\ensuremath{\tilde{\vg}}}
\newcommand{\gradestor}{\ensuremath{\hat{\vg}_{\vy}}}
\newcommand{\lambdaestor}{\ensuremath{\hat{\vlambda}}}
%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% parameter macros
\newcommand{\batchsizeone}{\ensuremath{K}}
\newcommand{\batchsizetwo}{\ensuremath{B}}
\newcommand{\samptrajlength}{\ensuremath{H}}
%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\pl}{PŁ\xspace}

\newcommand{\reinforce}{$\textsc{REINFORCE}$\xspace}
\newcommand{\hnabla}{\hat{\nabla}}


%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\regphi}{\Phi^\nu}


%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\hatg}{\hat{g}}
\newcommand{\sres}[1]{\hat{\vr}_\eta^{#1}}
\newcommand{\hatvg}{\hat{\vg}} 

\newcommand{\res}[1]{\vr_\eta^{#1}}
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\poly}{\mathsf{poly}}


\newcommand{\val}{V_{\vrho}}
\newcommand{\regval}{V_{\vrho}^\nu}
\newcommand{\sumactspa}{\sum_{i=1}^n|\calA_i| + |\calB|}
\newcommand{\diam}{\mathrm{Diam}}
\newcommand{\parsa}{\frac{\partial}{\partial x_{i,s,a}}}

\newcommand{\at}[1]{^{#1}}

==> table_online_learning.tex <==
\iffalse
\begin{table}[t]\label{table: online_learning}
\colorlet{hgh}{blue!20}
\centering
% \setlength{\tabcolsep}{16pt}
% \setlength\extrarowheight{6pt}
\begin{tabular}{p{2.65cm}lll}
  \rowcolors{2}{gray!25}{white}
% \hline

\textbf{Algorithm} & \textbf{Regret}  & \textbf{Feedback} & \textbf{Efficient}\color{blue}$^{\dagger}$ \\
\toprule


% Farina et al. \cite{farina2022kernelized}  &  $\widetilde{\mathcal{O}}\left(k^{3/2}\sqrt{T}\right)$  & Full-Info & \yes \\


% Farina et al. \cite{farina2022kernelized}  &  $\widetilde{\mathcal{O}}\left(m k^2\right)$  & Full-Info & \yes \\


% \hdashline


\color{black}{\textbf{This Work}}  & $\widetilde{\mathcal{O}}\left(k\sqrt{Td}\right)$  & Semi-Bandit & \yes \\

\hdashline

\citet{bartlett2008high}  & $\widetilde{\mathcal{O}}\left(d^{3/2}k\sqrt{T}\right)$  & {\color{blue}\no} \\

\citet{zero_suppressed}\newline Braun et al. \cite{braun2016efficientCOMBAND}  & $\widetilde{\mathcal{O}}\left(\left(\frac{k}{\sqrt{\lambda_{\text{min}}}} +  \frac{d\lambda_{\text{min}}}{k}\ \right) T^{2 / 3}\right)$ \color{blue}$^{\sharp}$  & \yes \\

Lee et al. \cite{bias_no_more} & $\widetilde{\mathcal{O}}\left(d^{7/2}k \sqrt{T}\right)$\color{blue}$^{^*}$  & \yes \\

Zimmert et al. \cite{zimmert2022returnLattimore}  & $\widetilde{\mathcal{O}}\left(dk\sqrt{T}\right)$  & {\color{blue}\no} \\


\color{black}{\textbf{This Work}} & $\mathcal{\widetilde{O}}\left(d^{2/3}k^{4/3}T^{2/3}\right)$   & \yes \\
\bottomrule

\end{tabular}
\caption{History of results with \textit{high probability guarantees} and \textit{adaptive adversaries}, eligible for online learning in combinatorial games. 
Regarding the semi-bandit setting, to the best of our knowledge, Algorithm \ref{alg:semi_band} is the first efficient general algorithm in the literature with high probability guarantees. 
{\color{blue}${\sharp}$}: We note that in Sakaue et al. \cite{zero_suppressed} and Braun et al. \cite{braun2016efficientCOMBAND}, $\lambda_{\text{min}}$ is the minimum eigenvector of the autocorrelation matrix under the law of the initial distribution $\mu$. 
$\lambda_{\text{min}}$ is possibly exponentially small in the general case. 
Common choices for $\mu$ include: (a) the uniform distribution ($\mu_{u}$) over the action space (as in \cite{zero_suppressed}) whose induced $\lambda_{\text{min}}$ can be difficult to bound in certain settings (e.g., see \cite{combinatorial_bandits, vu2019combinatorial}), or (b) the uniform distribution over an approximate barycentric spanner of the action space (as in \cite{braun2016efficientCOMBAND}), whose induced $\lambda_{\text{min}}$ can be also difficult to bound, because in general it is bounded from below by the minimum eigenvalue induced by $\mu_{u}$. 
{\color{blue}${*}$}: Although Lee et al. \cite{bias_no_more} provide regret guarantees only for continuous action spaces, their algorithm can be easily modified to incorporate regret guarantees for finite action sets via using an unbiased sample of the algorithm's $\widetilde{w}_t$. 
In the regime $T \leq d^{15}$, our regret bound is lower than that of \cite{bias_no_more}.
{\color{blue}${\dagger}$}: Efficient means that there exist combinatorial settings with finite actions in the literature where the respective algorithm can be implemented in time polylog($N$).}
\end{table}
\else
\begin{table}[htp]\label{table: online_learning}
\colorlet{hgh}{blue!20}
\centering
% \setlength{\tabcolsep}{16pt}
% \setlength\extrarowheight{6pt}
  % \rowcolors{2}{gray!25}{white}
\setlength{\tabcolsep}{4pt}
\scalebox{.87}{
\begin{tabular}{m{11mm}|m{2.68cm}ll}
% \hline

\bf Setting & \textbf{Algorithm} & \textbf{Regret}  & \hspace{-1.0cm}\textbf{Efficient}\color{blue}$^{\dagger}$ \\
\toprule


% Farina et al. \cite{farina2022kernelized}  &  $\widetilde{\mathcal{O}}\left(k^{3/2}\sqrt{T}\right)$  & Full-Info & \yes \\


% Farina et al. \cite{farina2022kernelized}  &  $\widetilde{\mathcal{O}}\left(m k^2\right)$  & Full-Info & \yes \\


% \hdashline


{Semi\newline Bandit} & \textcolor{black}{\textbf{This Work}}  & $\widetilde{\mathcal{O}}\left(\m\sqrt{Td}\right)$  & \yes \\

\hdashline
% \midrule

\multirow{4}{*}{\vspace*{-15mm}Bandit} & \cellcolor{gray!25}\citet{bartlett2008high}  & \cellcolor{gray!25}$\widetilde{\mathcal{O}}\left(d^{3/2}\m\sqrt{T}\right)$  & \cellcolor{gray!25}{\color{blue}\no} \\

& \citet{zero_suppressed}\newline Braun et al. \cite{braun2016efficientCOMBAND}  & $\widetilde{\mathcal{O}}\left(\left(\frac{\m}{\sqrt{\lambda_{\text{min}}}} +  \frac{d\lambda_{\text{min}}}{\m}\ \right) T^{2 / 3}\right)$\color{blue}$^{\sharp}$  & \yes \\

& \cellcolor{gray!25}Lee et al. \cite{bias_no_more} & \cellcolor{gray!25}$\widetilde{\mathcal{O}}\left(d^{7/2}\m \sqrt{T}\right)$\color{blue}$^{^*}$  & \cellcolor{gray!25}\yes \\

& Zimmert et al. \cite{zimmert2022returnLattimore}  & $\widetilde{\mathcal{O}}\left(d\m\sqrt{T}\right)$  & {\color{blue}\no} \\


& \cellcolor{gray!25}\color{black}{\textbf{This Work}} & \cellcolor{gray!25}$\mathcal{\widetilde{O}}\left(d^{2/3}\m^{4/3}T^{2/3}\right)$   & \cellcolor{gray!25}\yes \\
\bottomrule

\end{tabular}
}
\caption{Results with \textit{high probability guarantees} and \textit{adaptive adversaries}, eligible for online learning in combinatorial games.  
{\color{blue}${\sharp}$}: $\lambda_{\text{min}}$ is the minimum eigenvalue of the autocorrelation matrix of the initial distribution and can be exponentially small. 
{\color{blue}${*}$}: In the regime $T \leq d^{15}$, our regret bound is lower than that of \cite{bias_no_more}.
{\color{blue}${\dagger}$}: Efficient means that there exist combinatorial settings with finite actions in the literature where the respective algorithm can be implemented in time polylog($N$).}
\end{table}
\fi

 
% Common choices for $\mu$ include: (a) the uniform distribution ($\mu_{u}$) over the action space (as in \cite{zero_suppressed}) whose induced $\lambda_{\text{min}}$ can be difficult to bound in certain settings (e.g., see \cite{combinatorial_bandits, vu2019combinatorial}), or (b) the uniform distribution over an approximate barycentric spanner of the action space (as in \cite{braun2016efficientCOMBAND}), whose induced $\lambda_{\text{min}}$ can be also difficult to bound, because in general it is bounded from below by the minimum eigenvalue induced by $\mu_{u}$. 
